Symmetric Mass Generation as a Multicritical Point with Enhanced Symmetry

We explore the phase diagram of a lattice fermion model that exhibits three distinct phases: a massless fermion phase, a massive fermion phase with spontaneous symmetry breaking induced by a fermion bilinear condensate, and a massive fermion phase with symmetric mass generation. Using the fermion-bag Monte Carlo method on large cubical lattices, we find evidence for traditional second-order critical points separating the first two and the latter two phases. Remarkably, these critical points appear to merge at a multicritical point with enhanced symmetry when the symmetry breaking parameter is tuned to zero, giving rise to the recently discovered direct second-order transition between the massless and symmetric massive fermion phases.

==> header-1-packages.tex <==
\ifx\pdfsuppresswarningpagegroup\undefined\else\pdfsuppresswarningpagegroup=1\fi\relax
\RequirePackage{silence}
% We know this warning: Revtex does change \label, but fixes it for nameref as well
\WarningFilter{nameref}{The definition of \label has changed!}
% revtex will change the float package, OK, we are warned
\WarningFilter{revtex4-2}{Repair the float package}
\PassOptionsToPackage{unicode, pdfprintscaling=None, colorlinks}{hyperref}

% The curious construction is to unconfuse overleaf: it is simply the \documentclass command
\expandafter\relax\csname documentclass\endcsname[aps,prx,reprint,nofootinbib,preprintnumbers,floatfix,unsortedaddress,superscriptaddress,longbibliography]{revtex4-2}


\usepackage{orcidlink,multirow,siunitx,colortbl,dcolumn,tikz,graphicx,latexsym,amsmath,amssymb,amsfonts,bm,bbm,microtype,xspace,placeins,float,mathtools,xcolor,makecell,tabularx}

\usepackage[normalem]{ulem}
\usepackage[export]{adjustbox}
\usepackage{hyperref}
\usepackage[capitalise]{cleveref}

\usetikzlibrary{decorations.markings, arrows, decorations.pathmorphing}
\graphicspath{{pic/}}

\allowdisplaybreaks
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newlength{\FigureWidth}
\setlength{\FigureWidth}{3.3in}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\newcommand\TopRule{\Xhline{0.08em}}
\newcommand\HeaderRule{\Xhline{0.05em}}
\newcommand\MidRule{\Xhline{0.03em}}
\newcommand\BotRule{\Xhline{0.08em}}
\newcommand\SetTableProperties{
  \renewcommand{\arraystretch}{1.4}
}

\WarningFilter{revtex4-2}{Deferred float stuck}
\WarningFilter{latex}{A float is stuck}

\makeatletter
\newcommand\showtitleinbib{{\escapechar=`\\ \immediate\write\@auxout{%
\csname citation{REVTEX42Control}\endcsname^^J%
\csname citation{apsrev42Control}\endcsname
}}}
\makeatother

